The Parallax of Omega Centauri Measured from Gaia EDR3 and a Direct, Geometric Calibration of the Tip of the Red Giant Branch and the Hubble Constant

We use data from the ESA Gaia mission Early Data Release 3 (EDR3) to measure the trigonometric parallax of $\omega$ Cen, the first high precision parallax measurement for the most massive globular cluster in the Milky Way. We use a combination of positional and high quality proper motion data from EDR3 to identify over 100,000 cluster members, of which 67,000 are in the magnitude and color range where EDR3 parallaxes are best calibrated. We find the estimated parallax to be robust, demonstrating good control of systematics within the color-magnitude diagram of the cluster. We find a parallax for the cluster of $0.191\pm0.001$ (statistical) $\pm0.004$ (systematic) mas (2.2\% total uncertainty) corresponding to a distance of $5.24\pm0.11$ kpc. The parallax of $\omega$ Cen provides a unique opportunity to directly and geometrically calibrate the luminosity of the Tip of the Red Giant Branch (TRGB) because it is the only cluster with sufficient mass to provide enough red giant stars, more than 100 one magnitude below the tip, for a precise, model-free measurement of the tip. Combined with the pre-existing and most widely-used measurements of the tip and foreground Milky Way extinction, we find $M_{I,TRGB}=-3.97\pm0.06$ mag for the $I$-band luminosity of the blue edge. Using the TRGB luminosity calibrated from the Gaia EDR3 parallax of $\omega$ Cen to calibrate the luminosity of SNIa results in a value for the Hubble constant of $H_0=72.1\pm2.0$ km s$^{-1}$ Mpc$^{-1}$. We make the data for the stars in $\omega$ Cen available electronically and encourage independent analyses of the results presented here.

==> JournalAbbrevs.tex <==
\newcommand\aj{{AJ}}% 
          % Astronomical Journal 
\newcommand\araa{{ARA\&A}}% 
          % Annual Review of Astron and Astrophys 
%\newcommand\apj{{ApJ}}% 
          % Astrophysical Journal 
\newcommand\apjl{{ApJ}}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{{ApJS}}% 
          % Astrophysical Journal, Supplement 
%\newcommand\ao{{Appl.~Opt.}}% 
          % Applied Optics 
\newcommand\apss{{Ap\&SS}}% 
          % Astrophysics and Space Science 
\newcommand\aap{{A\&A}}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{{A\&A~Rev.}}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{{A\&AS}}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{{AZh}}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{{BAAS}}% 
          % Bulletin of the AAS 
\newcommand{\jcap}{J. Cosm. Astropart. Phys.}
	% Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{{JRASC}}% 
          % Journal of the RAS of Canada 
\newcommand\memras{{MmRAS}}% 
          % Memoirs of the RAS 
\newcommand\mnras{{MNRAS}}% 
          % Monthly Notices of the RAS 
%\newcommand\pra{{Phys.~Rev.~A}}% 
          % Physical Review A: General Physics 
%\newcommand\prb{{Phys.~Rev.~B}}% 
          % Physical Review B: Solid State 
%\newcommand\prc{{Phys.~Rev.~C}}% 
          % Physical Review C 
%\newcommand\prd{{Phys.~Rev.~D}}% 
          % Physical Review D 
%\newcommand\pre{{Phys.~Rev.~E}}% 
          % Physical Review E 
%\newcommand\prl{{Phys.~Rev.~Lett.}}% 
          % Physical Review Letters 
\newcommand\pasp{{PASP}}% 
          % Publications of the ASP 
\newcommand\pasj{{PASJ}}% 
          % Publications of the ASJ 
\newcommand\qjras{{QJRAS}}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{{S\&T}}% 
          % Sky and Telescope 
\newcommand\solphys{{Sol.~Phys.}}% 
          % Solar Physics 
\newcommand\sovast{{Soviet~Ast.}}% 
          % Soviet Astronomy 
\newcommand\ssr{{Space~Sci.~Rev.}}% 
          % Space Science Reviews 
\newcommand\zap{{ZAp}}% 
          % Zeitschrift fuer Astrophysik 
%\newcommand\nat{{Nature}}% 
          % Nature 
\newcommand\iaucirc{{IAU~Circ.}}% 
          % IAU Cirulars 
\newcommand\aplett{{Astrophys.~Lett.}}% 
          % Astrophysics Letters 
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{{Fund.~Cosmic~Phys.}}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{{Geophys.~Res.~Lett.}}% 
          % Geophysics Research Letters 
%\newcommand\jcp{{J.~Chem.~Phys.}}% 
          % Journal of Chemical Physics 
\newcommand\jgr{{J.~Geophys.~Res.}}% 
          % Journal of Geophysics Research 
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{{Nucl.~Phys.~A}}% 
          % Nuclear Physics A 
\newcommand\physrep{{Phys.~Rep.}}% 
          % Physics Reports 
\newcommand\physscr{{Phys.~Scr}}% 
          % Physica Scripta 
\newcommand\planss{{Planet.~Space~Sci.}}% 
          % Planetary Space Science 
\newcommand\procspie{{Proc.~SPIE}}% 
          % Proceedings of the SPIE 
\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 
